LifeTox: Unveiling Implicit Toxicity in Life Advice

As large language models become increasingly integrated into daily life, detecting implicit toxicity across diverse contexts is crucial. To this end, we introduce LifeTox, a dataset designed for identifying implicit toxicity within a broad range of advice-seeking scenarios. Unlike existing safety datasets, LifeTox comprises diverse contexts derived from personal experiences through open-ended questions. Experiments demonstrate that RoBERTa fine-tuned on LifeTox matches or surpasses the zero-shot performance of large language models in toxicity classification tasks. These results underscore the efficacy of LifeTox in addressing the complex challenges inherent in implicit toxicity. We open-sourced the dataset\footnote{\url{https://huggingface.co/datasets/mbkim/LifeTox}} and the LifeTox moderator family; 350M, 7B, and 13B.

==> Resources/vis2.tex <==
\begin{figure*}[bht]
\centering
\includegraphics[width=\textwidth]{Figures/vis2.pdf}
\caption{Visualization of Topic Distributions in \texttt{LifeTox}}
\label{fig:vis2}
\vspace{-5mm}
\end{figure*}
